Covariance Matrix Estimation for Massive MIMO

We propose a novel pilot structure for covariance matrix estimation in massive multiple-input multiple-output (MIMO) systems in which each user transmits two pilot sequences, with the second pilot sequence multiplied by a random phase-shift. The covariance matrix of a particular user is obtained by computing the sample cross-correlation of the channel estimates obtained from the two pilot sequences. This approach relaxes the requirement that all the users transmit their uplink pilots over the same set of symbols. We derive expressions for the achievable rate and the mean-squared error of the covariance matrix estimate when the proposed method is used with staggered pilots. The performance of the proposed method is compared with existing methods through simulations.

==> texFiles/pilotDecontamination.tex <==
\section{Mitigating Pilot Contamination Using the Trace of the Covariance Matrix}
\label{sec:pilotDecontamination}

In this subsection, we show that the ceiling on the UL rate due to pilot contamination (see \cite{Marzetta2010Noncooperative}) can be removed if the antenna arrays can be partitioned into subsets such that the traces of the covariance matrices in each of the subsets can be arranged in a non-singular matrix. It has been shown in \cite{bjornson2017unlimited} that the diagonals of the covariance matrices are sufficient for eliminating the ceiling on the UL rate. This result is useful since estimating the diagonal requires far less resources than estimating the whole covariance matrix. However, our approach requires a significantly smaller overhead since estimating the trace of a covariance matrix requires fewer observations than estimating either the diagonal or the whole covariance matrix. 
 
Consider a multi-cell multi-user scenario with the $ \vIdxTwo\rth $ user of the $ \sIdxOne\rth $ cell having the channel $ \mbf{h}_{\sIdxOne} $ with corresponding covariance matrix $ \mbf{R}_{\sIdxOne} $ at the BS of cell $ \vIdxOne $. The subscripts $ \vIdxOne $ and $ \vIdxTwo $ have been dropped from $ \mbf{h}_{\sIdxOne} $ and $ \mbf{R}_{\sIdxOne} $ for the sake of simplicity. Then, we have the following lemma.
\begin{lemma}
	\label{lemma}
	If the $ M $ antennas at the BS can be divided into $ L $ subsets $ \mathcal{S}_{\sIdxOne} $ each containing $ \alpha_{\sIdxOne} M $ antennas (where $ \alpha_{\sIdxOne} > 0 $ and $ \sum\limits_{\sIdxOne}\alpha_{\sIdxOne} = 1 $), the achievable rate increases linearly in $ M $ if the subsets $ \mathcal{S}_{\sIdxOne} $ are chosen such that the matrix
	\begin{align}
		\mbf{T}
		\triangleq
		\begin{bmatrix}
		r_{00} & \ldots & r_{L-1,0}\\
		r_{01} &\ldots &r_{L-1,1} \\
		 \vdots&\ddots&\vdots\\
		r_{0,L-1}&\ldots &r_{L-1,L-1} \\
		\end{bmatrix}
	\end{align}
	is non-singular, where $ r_{\sIdxOne\sIdxThree}\triangleq \mathrm{trace}\lrf{\mbf{R}_{\sIdxOne\sIdxThree}}/|\mathcal{S}_{\sIdxThree}| $ and the matrix $ \mbf{R}_{\sIdxOne\sIdxThree} $ is the covariance matrices of the user in cell $ \sIdxOne $ for antenna subset $ \mathcal{S}_{\sIdxThree} $.
	\begin{proof}
		For the case where each cell has only a single-user sharing a common pilot\footnote{The interference from users that share different pilots goes to zero asymptotically in $ M $ \cite{Marzetta2010Noncooperative}.} the received observation vector $ \mbf{y}_{\sIdxThree} $ corresponding to antenna subset $ \mathcal{S}_{\sIdxThree} $ can be written as
		\begin{align}
			\mbf{y}_{\sIdxThree} = \sum\limits_{\sIdxOne} \mbf{h}_{\sIdxOne\sIdxThree} x_{\sIdxOne} + \mbf{w}_{\sIdxThree}
		\end{align}
		where $ \mbf{h}_{\sIdxOne\sIdxThree} $ is the channel vector of the user in cell $ \sIdxOne $ in antenna subset $ \mathcal{S}_{\sIdxThree} $.
		Using the LS estimate of the channel $ \widehat{\mbf{h}}_{00} $ in a matched filter, the estimate of the data of the reference user $ 0 $ can be obtained from antenna subset $ \mathcal{S}_{0} $ as
		\begin{align}
			\widehat{x}_{00} 
			&= \frac{1}{|\mathcal{S}_0|} \widehat{\mbf{h}}_{00}^H \lrc{\sum\limits_{\sIdxOne} \mbf{h}_{\sIdxOne 0} x_{\sIdxOne} + \mbf{w}_{0}}\nonumber\\
			&= 
			\frac{\mathrm{trace}\lrf{\mbf{R}_{0 0}}}{|\mathcal{S}_0|} x_{0} 
			+
			\sum\limits_{\sIdxOne\neq 0}
			\frac{\mathrm{trace}\lrf{\mbf{R}_{\sIdxOne 0}}}{|\mathcal{S}_0|} x_{\sIdxOne} 
			+ 
			i_{0}
			\label{eqn:antennaSubset0MfOutput}
			\\
			i_0 &\triangleq
			\sum\limits_{\sIdxOne}
			\lrc{\frac{\widehat{\mbf{h}}_{00}^H\mbf{h}_{\sIdxOne0}}{|\mathcal{S}_0|}-\frac{\mathrm{trace}\lrf{\mbf{R}_{\sIdxOne 0}}}{|\mathcal{S}_0|}} x_{\sIdxOne} + \mbf{w}_{0}
			\label{eqn:antennaSubset0Interference}\;.
		\end{align}
		It can be observed that the first term in \eqref{eqn:antennaSubset0MfOutput} is uncorrelated with the second and third terms.	
		Using the similar approach as above, $ \widehat{x}_{0\sIdxThree}\;\forall \sIdxThree $ can be obtained. Then, we can write
		${
			\widehat{\mbf{x}}_0
			=
			\mbf{T}
			\mbf{x}
			+
			\mbf{i}}
		$,
		where $ {\widehat{\mbf{x}}_0 \triangleq \lrs{\widehat{x}_{00}, \ldots,\widehat{x}_{0,L-1}}^T} $, $ {\mbf{x} \triangleq \lrs{x_0,\ldots,x_{L-1}}^T} $ and $ \mbf{i} = \lrs{i_0,\ldots,i_{L-1}}^T $. Now, if $ \mbf{T} $ is non-singular, an estimate of $ x_0 $ can be obtained as
		\begin{align}
			\widehat{x}_0 &= \mbf{e}_1^T \mbf{T}^{-1} 	
			\widehat{\mbf{x}}_0
			=
			x_0
			+
			\mbf{e}_1^T \mbf{T}^{-1}
			\mbf{i}
			\label{eqn:estimateX0}
		\end{align}
		where $ \mbf{e}_1 $ is the first column of $ \eye_{L} $. The interference term $ \mbf{e}_1^T \mbf{T}^{-1}\mbf{i} $ in \eqref{eqn:estimateX0} is uncorrelated with $ x_0 $ and its variance decreases linearly in $ M $. Therefore replacing $ \mbf{e}_1^T \mbf{T}^{-1}\mbf{i} $ with Gaussian noise of the same variance, a lower bound on the SINR can be obtained as in \cite{Hassibi2003HowMuch}. This bound on the SINR increases linearly in $ M $.
	\end{proof}
\end{lemma}
A interesting consequence of Lemma \ref{lemma} is that only the trace of the covariance matrices in particular subsets are sufficient to design a data combiner that will result in an asymptotic increase in the UL rate. However, the approach detailed in Lemma \ref{lemma} is contingent on finding the subsets $ \mathcal{S}_{\sIdxThree} $. Efficient selection of the subsets $ \mathcal{S}_{\sIdxThree} $, such that the matrix $ \mbf{T} $ would be non-singular, is a problem will need to be addressed for any practical scenario.
